TESSERACT: Gradient Flip Score to Secure Federated Learning Against Model Poisoning Attacks

Federated learning---multi-party, distributed learning in a decentralized environment---is vulnerable to model poisoning attacks, even more so than centralized learning approaches. This is because malicious clients can collude and send in carefully tailored model updates to make the global model inaccurate. This motivated the development of Byzantine-resilient federated learning algorithms, such as Krum, Bulyan, FABA, and FoolsGold. However, a recently developed untargeted model poisoning attack showed that all prior defenses can be bypassed. The attack uses the intuition that simply by changing the sign of the gradient updates that the optimizer is computing, for a set of malicious clients, a model can be diverted from the optima to increase the test error rate. In this work, we develop TESSERACT---a defense against this directed deviation attack, a state-of-the-art model poisoning attack. TESSERACT is based on a simple intuition that in a federated learning setting, certain patterns of gradient flips are indicative of an attack. This intuition is remarkably stable across different learning algorithms, models, and datasets. TESSERACT assigns reputation scores to the participating clients based on their behavior during the training phase and then takes a weighted contribution of the clients. We show that TESSERACT provides robustness against even a white-box version of the attack.

==> sections/reserve.tex <==
\begin{table}[]
\begin{minipage}[c]{0.5\linewidth}
    \begin{comment}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Attack & \multicolumn{2}{c|}{FoolsGold} & \multicolumn{2}{c|}{FLTrust} \\
        \hline
        {} & Mal & Ben & Mal & Ben \\
        \hline
        Benign & - & 0.29 & - & 0.48\\
        \hline
        Full-Trim & 0.00 & 0.30 & 0.52 & 0.45\\
        \hline
        Full-Krum & 0.64 & 0.10 & 0.63 & 0.49\\
        \hline
    \end{tabular}
    \end{comment}
    \centering
    \begin{tabular}{|c|c|c|c|}
        \hline
        Defense & Benign & Full-trim & Full-krum \\
        \hline
        FoolsGold (Mal) & Mal & Ben & Mal \\
        \hline
        FoolsGold (Ben) & - & 0.29 & \\
        \hline
        FLtrust (Mal) & 0.00 & 0.30 & 0.52\\
        \hline
        FLTrust (Ben) & 0.64 & 0.10 & 0.63\\
        \hline
        \name (Mal) & & &  \\
        \hline
        \name (Ben) & & & \\
        \hline
    \end{tabular}    
\end{minipage} 
\begin{minipage}[c]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{iclr2022/figures/reputation.png}
    \label{fig:reputation}
\end{minipage}
\begin{comment}
\begin{minipage}[c]{0.5\linewidth}
    \centering
    \begin{tabular}{|c|c|c|}
        \hline
        Attack & \multicolumn{2}{c|}{\name}  \\
        \hline
        {} & Mal & Ben \\
        \hline
        Benign & - & 0.75\\
        \hline
        Full-Trim & 0.00 & 0.82\\
        \hline
        Full-Krum & 0.09 & 0.73\\
        \hline
    \end{tabular}
\end{minipage} 
\end{comment}
\caption{Average number of malicious or benign clients that were allotted non-zero weights by FoolsGold and FLTrust during training, normalized by the total number of malicious and benign clients respectively. We can see that in every iteration, more than half of the benign clients were {\em not} allowed to contribute to the global model update. In \name, the proportions for benign clients are higher, indicating that fewer false positive errors. Conversely, the proportions for malicious clients are lower in \name than baselines, indicating it penalizes malicious clients more.}
\label{tab:filter}
\end{table}

\begin{figure}
\begin{minipage}[c]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{iclr2022/figures/reputation.png}
    \label{fig:reputation}
\end{minipage}
\begin{minipage}[c]{0.5\linewidth}
    \centering
    \includegraphics[width=\textwidth]{}
    \label{fig:faba}
\end{minipage}
\caption{}
\end{figure}
